Conceptual structure and the growth of scientific knowledge

How does scientific knowledge grow? This question has occupied a central place in the philosophy of science, stimulating heated debates, but yielding no clear consensus. Many explanations can be understood in terms of whether and how they view the expansion of knowledge as proceeding through the accretion of scientific concepts into larger conceptual structures. Here, we examine these views empirically, performing a large-scale analysis of the physical and social sciences, spanning five decades. Using natural language processing techniques, we create semantic networks of concepts, wherein noun phrases become linked when used in the same paper abstract. For both the physical and social sciences, we observe increasingly rigid conceptual cores (i.e., densely connected sets of highly central nodes) accompanied by the proliferation of periphery concepts (i.e., sparsely connected nodes that are highly connected to the core). Subsequently, we examine the relationship between conceptual structure and the growth of scientific knowledge, finding that scientific works are more innovative in fields with cores that have higher conceptual churn and with larger cores. Furthermore, scientific consensus is associated with reduced conceptual churn and fewer conceptual cores. Overall, our findings suggest that while the organization of scientific concepts is important for the growth of knowledge, the mechanisms vary across time.

==> commands.tex <==

% blackboard bold for naturals, integers, etc.
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}

%comments shown

\newcommand{\russ}[1]{\textcolor{orange}{(Russ says: {#1})}}
\newcommand{\kara}[1]{\textcolor{blue}{(Kara says: {#1})}}
\newcommand{\ekaterina}[1]{\textcolor{red}{(Ekaterina says: {#1})}}

\newcommand{\beginsupplement}{%
        \setcounter{table}{0}
        \renewcommand{\thetable}{S\arabic{table}}%
        \setcounter{figure}{0}
        \renewcommand{\thefigure}{S\arabic{figure}}%
     }


% text commands
\newcommand{\mc}{\mathcal}
\newcommand{\mb}{\mathbb}
\newcommand{\mf}{\mathfrak}
\newcommand{\tn}[1]{\textnormal{#1}}


% greek lower case
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\g}{\gamma}
\renewcommand{\d}{\delta}
\newcommand{\e}{\varepsilon}
\newcommand{\w}{\omega}
\newcommand{\s}{\sigma}
\newcommand{\ph}{\varphi}
\newcommand{\p}{\partial}
\renewcommand{\t}{\tau}
\renewcommand{\th}{\theta}
\newcommand{\z}{\zeta}

% greek upper case
\newcommand{\Om}{\Omega}
\newcommand{\Ga}{\Gamma}
\newcommand{\Si}{\Sigma}
\newcommand{\La}{\Lambda}

% script upper case
\newcommand{\A}{\mathscr{A}}
\newcommand{\B}{\mathscr{B}}


%% counter for labels in description env
\newcounter{desccount}
\newcommand{\descitem}[1]{%
  \item[#1] \refstepcounter{desccount}\label{#1}
}
\newcommand{\descref}[1]{\hyperref[#1]{#1}}


% pullback functions
\newcommand{\fst}{f^{*}}
\newcommand{\gst}{g^{*}}


% misc

\newcommand{\uniflim}{\operatorname{unif}\lim}
\newcommand{\unifr}{\xrightarrow{\operatorname{unif.}}}

\renewcommand{\P}{\mathbb{P}}
\newcommand{\hr}{\hookrightarrow}
\newcommand{\li}{\lambda_I}
\newcommand{\lp}{\left(}
\newcommand{\rp}{\right)}
\newcommand{\lbar}{\left|}
\newcommand{\rbar}{\right|}
\newcommand{\lnorm}{\left\|}
\newcommand{\rnorm}{\right\|}

\newcommand\mattwo[4]{\left(\begin{smallmatrix}
			{#1} & {#2}\\
     			{#3} & {#4}
                     \end{smallmatrix}\right)}
\newcommand\mattres[9]{\left(\begin{smallmatrix}
			{#1} & {#2}&{#3}\\
     			{#4} & {#5}&{#6}\\
     				{#7} &{#8} &{#9}
                     \end{smallmatrix}\right)}
                     
\newcommand{\linf}{l^{\infty}}		%l-infinity norm
\newcommand{\borel}{\operatorname{Borel}}	
\newcommand{\fa}{\forall}
\newcommand{\set}[1]{\left\{#1\right\}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\ip}[2]{\left\la #1,#2 \right\ra}
\renewcommand{\o}{\overline}
\renewcommand{\u}{\underline}
\newcommand{\h}{\hat}
\renewcommand{\r}{\rightarrow}
\newcommand{\xr}{\xrightarrow}
\newcommand{\pa}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\de}[2]{\frac{d #1}{d #2}}
\newcommand{\ddx}{\frac{d}{dx}}
\newcommand{\norm}[1]{\|#1\|} 
\newcommand{\tnorm}[1]{||#1||} % two-norm, i.e., with two bars
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\newcommand{\rw}{\rightharpoonup}
\renewcommand{\emptyset}{\varnothing}
\newcommand{\pair}[1]{\left(#1\right)}
\newcommand{\supp}{\operatorname{supp}}
\newcommand{\wh}{\widehat}
\renewcommand{\div}{\operatorname{div}}
\newcommand{\diam}{\operatorname{diam}}
\newcommand{\pv}{\operatorname{PV}}
\newcommand{\curl}{\operatorname{curl}}
\newcommand{\ds}{\displaystyle}
\newcommand{\inv}{^{-1}}
\newcommand{\dg}[1]{\textnormal{deg(#1)}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\ind}{\operatorname{Ind}}
\newcommand{\im}{\operatorname{im}}

%% In an integral, for the differential term
%\newcommand*\diff{\mathop{}\!\mathrm{d}}
\newcommand{\diff}{\, d}
%% For denoting powers of a differential term
\newcommand*\Diff[1]{\mathop{}\!\mathrm{d^#1}}

%% integral with space removed
\newcommand{\myint}{\int\!}

\newcommand{\ceil}[1]{\left \lceil{#1}\right \rceil }
\newcommand{\floor}[1]{\left \lfloor{#1}\right \rfloor }


%% PH stuff?
\newcommand{\pathhom}{\mathbf{PathHom}}
\newcommand{\dfchom}{\mathbf{DFCHom}}

\newcommand{\mlp}[1]{K^{\rightarrow}_{n_1,\ldots,n_{#1}}} 
\newcommand{\mlpgraph}[1]{K_{n_1,\ldots,n_{#1}}} 


\newcommand{\db}{d_{\operatorname{B}}}
\newcommand{\dgm}{\operatorname{Dgm}}
\newcommand{\vr}{\operatorname{VR}}
\newcommand{\cech}{\check{\operatorname{C}}}
\newcommand{\pvec}{{\operatorname{\mathbf{PVec}}}}
\newcommand{\pers}{{\operatorname{\mathbf{Pers}}}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\di}{d_{\operatorname{I}}}

\newcommand{\src}{\mf{D}^{\operatorname{so}}}
\newcommand{\sink}{\mf{D}^{\operatorname{si}}}

\newcommand{\so}{\operatorname{so}}
\newcommand{\si}{\operatorname{si}}



\newtheorem{theorem}{Theorem}
\newtheorem{question}{Question}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}


\theoremstyle{definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{defn}{Definition}
\newtheorem{definition}{Definition}
\newtheorem{claim}{Claim}
\newtheorem*{comments}{Comments}
%

\newenvironment{subproof}[1][\proofname]{%
  \renewcommand{\qedsymbol}{$\blacksquare$}%
  \begin{proof}[#1]%
}{%
  \end{proof}%
}

%% for align right within equation
\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother



==> packages.tex <==


%\usepackage{arxiv}

\usepackage{booktabs} 
\usepackage{nicefrac}  
\usepackage{microtype}
\usepackage[utf8]{inputenc}

%\usepackage{enumitem}
%\usepackage{times}
%\usepackage{amsaddr}
%\usepackage[margin=1in]{geometry}

% \usepackage[dvipsnames]{xcolor}
\usepackage{wrapfig}
% \usepackage{multirow}

%\usepackage{url}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{bbm}
%\usepackage[normalem]{ulem}
%\usepackage{mathabx}
\usepackage{bbm}
\usepackage{array}
\usepackage[colorlinks=true,urlcolor=purple,
linkcolor=purple,citecolor=purple]{hyperref}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{float}

% tables and figures
\usepackage{lscape}
\usepackage{graphicx}

% for nicer tables
\usepackage{booktabs}
\usepackage{longtable}
% \usepackage[skip=0pt, font=sc]{caption}
\usepackage{threeparttable}
\usepackage{threeparttablex}
% \usepackage[capposition=top]{floatrow}


\usepackage{mathrsfs}
%\usepackage{framed}
%\usepackage{latexsym}
%\usepackage{pb-diagram}
%\usepackage[mathscr]{}
\usepackage{graphicx}
%\usepackage[all]{xy} 
\usepackage{color}
\usepackage{natbib}

\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{thmtools,thm-restate} %%for restating results 
%\usepackage[usenames, dvipsnames]{color}

\makeatletter
\def\paragraph{\@startsection{paragraph}{4}%
  \z@\z@{-\fontdimen2\font}%
  {\normalfont\bfseries}}
\makeatother

%% TIK-Z RELATED PACKAGES
\usepackage{tikz}
\usetikzlibrary{decorations.markings, backgrounds, calc, positioning, shapes, shadows, arrows, fit, automata}
\usepackage{tikz-cd}
% Nice arrowheads
\usetikzlibrary{arrows.meta}
%\tikzset{>={Latex[length=3mm,width=2mm]}}
\tikzset{>={Latex}}



==> table_consensus_regressions.tex <==
 
                                             &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   \\
\midrule
$\textit{C}\textsubscript{it}$: Churn of core nodes&        -1.4168** &        -1.3840** \\
                                             &       (0.4502)   &       (0.4582)   \\
$\textit{R}\textsubscript{it}$: No. of core nodes (\%)&         0.0025   &         0.0010   \\
                                             &       (0.0031)   &       (0.0031)   \\
$\textit{S}\textsubscript{it}$: No. of cores &        -0.0009** &        -0.0007*  \\
                                             &       (0.0004)   &       (0.0004)   \\
No. of nouns in abstract (log)               &        -0.1720***&        -0.1873***\\
                                             &       (0.0240)   &       (0.0244)   \\
No. of adjectives in abstract (log)          &         0.5254***&         0.5227***\\
                                             &       (0.0217)   &       (0.0222)   \\
No. of verbs in abstract (log)               &        -0.0260   &        -0.0194   \\
                                             &       (0.0266)   &       (0.0269)   \\
No. of adverbs in abstract (log)             &         0.1889***&         0.1908***\\
                                             &       (0.0140)   &       (0.0142)   \\
No. of authors                               &                  &         0.0024   \\
                                             &                  &       (0.0024)   \\
No. of references                            &                  &         0.0112***\\
                                             &                  &       (0.0010)   \\
Constant                                     &        -0.7697** &        -0.8276***\\
                                             &       (0.2375)   &       (0.2414)   \\\midrule
Field fixed effects                          &            Yes   &            Yes   \\
Year fixed effects                           &            Yes   &            Yes   \\
\midrule
N                                            &          80599   &          79669   \\
Mcfadden's pseudo-R2                         &           0.02   &           0.02   \\
 


==> table_outcomes_regressions.tex <==
 
                                             &\multicolumn{2}{c}{\shortstack{Physical Sciences}}&\multicolumn{2}{c}{\shortstack{Social Sciences}}\\\cmidrule(lr){2-3}\cmidrule(lr){4-5}
                                             &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   &\multicolumn{1}{c}{(3)}   &\multicolumn{1}{c}{(4)}   \\
\midrule
$\textit{C}\textsubscript{it}$: Churn of core nodes&         0.0476***&         0.0471***&         0.0265***&         0.0196** \\
                                             &       (0.0087)   &       (0.0088)   &       (0.0081)   &       (0.0079)   \\
$\textit{R}\textsubscript{it}$: No. of core nodes (\%)&         0.0006***&         0.0006***&         0.0027***&         0.0032***\\
                                             &       (0.0001)   &       (0.0001)   &       (0.0001)   &       (0.0001)   \\
$\textit{S}\textsubscript{it}$: No. of cores (log)&        -0.0150***&        -0.0170***&        -0.0097***&        -0.0134***\\
                                             &       (0.0021)   &       (0.0021)   &       (0.0014)   &       (0.0014)   \\
No. of authors                               &                  &        -0.0010***&                  &        -0.0040***\\
                                             &                  &       (0.0001)   &                  &       (0.0001)   \\
No. of references                            &                  &        -0.0014***&                  &        -0.0026***\\
                                             &                  &       (0.0000)   &                  &       (0.0000)   \\
Field fixed effects                          &            Yes   &            Yes   &            Yes   &            Yes   \\
Year fixed effects                           &            Yes   &            Yes   &            Yes   &            Yes   \\
\midrule
N                                            &         438374   &         432079   &        1768191   &        1768110   \\
Adjusted R2                                  &           0.02   &           0.03   &           0.06   &           0.10   \\
\midrule Wald tests for core/periphery predictors&                  &                  &                  &                  \\
F                                            &          73.86   &          88.42   &        1078.06   &        1722.96   \\
d.f.                                         &           3.00   &           3.00   &           3.00   &           3.00   \\
p-value                                      &           0.00   &           0.00   &           0.00   &           0.00   \\\bottomrule
 


==> table_random_network_adjusted_regressions_B2_rr2.tex <==
 
                                             &\multicolumn{1}{c}{\shortstack{Social Sciences}}&\multicolumn{1}{c}{\shortstack{Physical Sciences}}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}
                                             &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   \\
\midrule
$\textit{C}\textsubscript{it}$: Churn of core nodes (Observed Network)&         0.2055*  &         0.1953***\\
                                             &       (0.0800)   &       (0.0424)   \\
$\textit{R}\textsubscript{it}$: No. of core nodes (\%) (Observed Network)&         0.0047***&         0.0009** \\
                                             &       (0.0005)   &       (0.0003)   \\
$\textit{S}\textsubscript{it}$: No. of cores (Observed Network)&        -0.0002*  &        -0.0000   \\
                                             &       (0.0001)   &       (0.0000)   \\
$\textit{C}\textsubscript{it}$: Churn of core nodes (Random Network)&         0.0606   &        -0.0099   \\
                                             &       (0.0851)   &       (0.0344)   \\
$\textit{R}\textsubscript{it}$: No. of core nodes (\%) (Random Network)&         0.0010   &        -0.0003   \\
                                             &       (0.0005)   &       (0.0003)   \\
$\textit{S}\textsubscript{it}$: No. of cores (Random Network)&         0.0005***&         0.0000   \\
                                             &       (0.0001)   &       (0.0000)   \\
No. of authors                               &        -0.0042***&        -0.0010***\\
                                             &       (0.0003)   &       (0.0001)   \\
No. of references                            &        -0.0026***&        -0.0015***\\
                                             &       (0.0003)   &       (0.0001)   \\
Field fixed effects                          &            Yes   &            Yes   \\
Year fixed effects                           &            Yes   &            Yes   \\
\midrule
N                                            &       8.83e+07   &       2.08e+07   \\
Adjusted R2                                  &           0.11   &           0.03   \\
\midrule Wald tests for core/periphery predictors&                  &                  \\
F                                            &          28.24   &          10.28   \\
d.f.                                         &           3.00   &           3.00   \\
p-value                                      &           0.00   &           0.00   \\
 


==> table_random_network_regressions_zscores_B2_rr2.tex <==
 
                                             &\multicolumn{1}{c}{\shortstack{Social Sciences}}&\multicolumn{1}{c}{\shortstack{Physical Sciences}}\\\cmidrule(lr){2-2}\cmidrule(lr){3-3}
                                             &\multicolumn{1}{c}{(1)}   &\multicolumn{1}{c}{(2)}   \\
\midrule
$\textit{C}\textsubscript{it}$: Churn of core nodes (Comparative Index)&         0.0034***&         0.0025***\\
                                             &       (0.0002)   &       (0.0004)   \\
$\textit{R}\textsubscript{it}$: No. of core nodes (\%) (Comparative Index)&         0.0014***&         0.0022***\\
                                             &       (0.0002)   &       (0.0003)   \\
$\textit{S}\textsubscript{it}$: No. of cores (Comparative Index)&         0.0058***&        -0.0010   \\
                                             &       (0.0002)   &       (0.0006)   \\
No. of authors                               &        -0.0040***&        -0.0009***\\
                                             &       (0.0001)   &       (0.0001)   \\
No. of references                            &        -0.0025***&        -0.0015***\\
                                             &       (0.0000)   &       (0.0000)   \\
Field fixed effects                          &            Yes   &            Yes   \\
Year fixed effects                           &            Yes   &            Yes   \\
\midrule
N                                            &        1765682   &         416294   \\
Adjusted R2                                  &           0.10   &           0.03   \\
\midrule Wald tests for core/periphery predictors&                  &                  \\
F                                            &         366.89   &          28.55   \\
d.f.                                         &           3.00   &           3.00   \\
p-value                                      &           0.00   &           0.00   \\
 

